Categories of Differentiable Polynomial Circuits for Machine Learning

Reverse derivative categories (RDCs) have recently been shown to be a suitable semantic framework for studying machine learning algorithms. Whereas emphasis has been put on training methodologies, less attention has been devoted to particular \emph{model classes}: the concrete categories whose morphisms represent machine learning models. In this paper we study presentations by generators and equations of classes of RDCs. In particular, we propose \emph{polynomial circuits} as a suitable machine learning model. We give an axiomatisation for these circuits and prove a functional completeness result. Finally, we discuss the use of polynomial circuits over specific semirings to perform machine learning with discrete values.

==> Makefile <==
OUT := build
BIB := main.bib

BUILD_CMD := xelatex -interaction=nonstopmode -output-directory $(OUT)

all: pdf bib

$(OUT):
	mkdir -p $(OUT)

pdf: main.tex $(OUT)
	$(BUILD_CMD) main.tex

bib: *.bib
	cat *.bib > $(OUT)/main.bib
	if [ -s $(OUT)/main.bib ]; then \
		set -e; cd $(OUT); bibtex main; \
	fi

view:
	zathura build/main.pdf &

